HD-OOD3D: Supervised and Unsupervised Out-of-Distribution object detection in LiDAR data

Autonomous systems rely on accurate 3D object detection from LiDAR data, yet most detectors are limited to a predefined set of known classes, making them vulnerable to unexpected out-of-distribution (OOD) objects. In this work, we present HD-OOD3D, a novel two-stage method for detecting unknown objects. We demonstrate the superiority of two-stage approaches over single-stage methods, achieving more robust detection of unknown objects while addressing key challenges in the evaluation protocol. Furthermore, we conduct an in-depth analysis of the standard evaluation protocol for OOD detection, revealing the critical impact of hyperparameter choices. To address the challenge of scaling the learning of unknown objects, we explore unsupervised training strategies to generate pseudo-labels for unknowns. Among the different approaches evaluated, our experiments show that top-5 auto-labelling offers more promising performance compared to simple resizing techniques.

==> tab/eval_subset_setting_new.tex <==
\begin{comment}
    
\begin{table}[ht]
\centering
\scalebox{0.7}{
\begin{tabular}{|c|||c||c|c|c|c|}%c|}
\hline
Evaluation Subset & Method & AUROC $\uparrow$ & FPR-95 $\downarrow$&  AUPR-E $\uparrow$ & AUPR-S  $\uparrow$ \\%& AP $\uparrow$\\
\hline
\hline
%& MaxLogit &  76.2&  85.2&  2.5&  98.7&  \\
\multirow{3}{*}{All Scans}  & MaxSoftMax & 87.7 & 67.2 & 5.9 & 96.7\\%&  \\
 & Energy & 66.8&94.6&1.6&99.4\\%&  \\
% & Default Score& 78.6&84.3&2.8&99.7&\\
% & Monte Carlo Dropout\todo{} &  &  &  &  &  \\
\cline{2-6}
 & Real unknown instances (Pooling) & 88.5 & 51.5&9.4&99.8\\%&  \\
% & Real unknown instances (Like Paper) \todo{}&  &  &  &  &  \\
\hline
%& MaxLogit &  75.3&  85.7& 4.0 & 98.5 &  \\
\multirow{3}{*}{"Open" Scans}  & MaxSoftMax&83.7&74.1&7.1&97.5\\%& \\
 & Energy &66.1&91.9&2.6&99.1\\%&\\
% & Default Score&75.9&84.9&4.2&99.4& \\
% & Monte Carlo Dropout \todo{}&  &  &  &  &  \\
\cline{2-6}
 & Real unknown instances (Pooling) &88.1 & 51.0 & 15.2& 99.7\\%& \\
% & Real unknown instances (Like Paper)& 88.9 & 49.2& 16.7& 71.4& \\
\hline
\end{tabular}}
\caption{Impact of using a subset of evaluation set containing open class instances on OOD Metrics for Open and Closed Ground Truth Objects in the Argoverse2 Dataset}
\label{tab:eval_subset_setting}
\end{table}
\end{comment}

\begin{comment}
    
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l | l | c c c c }%c|}
%\hline
Evaluation Subset & Method & AUROC $\uparrow$ & FPR-95 $\downarrow$&  AUPR-E $\uparrow$ & AUPR-S  $\uparrow$ \\%& AP $\uparrow$\\
\hline
%& MaxLogit &  76.2&  85.2&  2.5&  98.7&  \\
\multirow{2}{*}{All Scans}  & 1-stage: MaxSoftMax & 87.7 & 67.2 & 5.9 & 96.7\\%&  \\
% & Energy & 66.8&94.6&1.6&99.4\\%&  \\
% & Default Score& 78.6&84.3&2.8&99.7&\\
% & Monte Carlo Dropout\todo{} &  &  &  &  &  \\
%\cline{2-6}
 & 2-stage: oracle MLP  $\dagger$ & 88.5 & 51.5& \textbf{9.4}&99.8\\%&  \\
% & Real unknown instances (Like Paper) \todo{}&  &  &  &  &  \\
\hline
%& MaxLogit &  75.3&  85.7& 4.0 & 98.5 &  \\
\cellcolor{gray!20}  & \cellcolor{gray!20}1-stage: \cellcolor{gray!20}MaxSoftMax &\cellcolor{gray!20}83.7&\cellcolor{gray!20}74.1&\cellcolor{gray!20}7.1&\cellcolor{gray!20}97.5\\%& \\
% & Energy &66.1&91.9&2.6&99.1\\%&\\
% & Default Score&75.9&84.9&4.2&99.4& \\
% & Monte Carlo Dropout \todo{}&  &  &  &  &  \\
%\cline{2-6}
\multirow{-2}{*}{\cellcolor{gray!20}"Open" Scans} & \cellcolor{gray!20}2-stage: oracle MLP $\dagger$ &\cellcolor{gray!20}88.1 & \cellcolor{gray!20}51.0 & \cellcolor{gray!20}\textbf{15.2}& \cellcolor{gray!20}99.7\\%& \\
% & Real unknown instances (Like Paper)& 88.9 & 49.2& 16.7& 71.4& \\
%\hline
\end{tabular}
}
\caption{Impact on the OOD results of the choice of the evaluation set in Argoverse 2 dataset ($\dagger$ means that the 2-stage MLP uses the annotation of unknown classes for its training). \todo{Test JE}}
\label{tab:eval_subset_setting_test_JE}
\end{table}
\end{comment}

\begin{comment}
    
\end{comment}
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l | l | c c c c }%c|}
Evaluation Subset & Method & AUROC $\uparrow$ & FPR-95 $\downarrow$&  AUPR-E $\uparrow$ & AUPR-S  $\uparrow$ \\%& AP $\uparrow$\\
\hline
\multirow{2}{*}{All Scans}  & 1-stage: MaxSoftMax & 87.7 & 67.2 & 5.9 & 96.7\\
 & 2-stage: oracle MLP  $\dagger$ & 88.5 & 51.5& \textbf{9.4}&99.8\\
\hline
\cellcolor{gray!20}  & \cellcolor{gray!20}1-stage: \cellcolor{gray!20}MaxSoftMax &\cellcolor{gray!20}83.7&\cellcolor{gray!20}74.1&\cellcolor{gray!20}7.1&\cellcolor{gray!20}97.5\\
\multirow{-2}{*}{\cellcolor{gray!20}"Open" Scans} & \cellcolor{gray!20}2-stage: oracle MLP $\dagger$ &\cellcolor{gray!20}88.1 & \cellcolor{gray!20}51.0 & \cellcolor{gray!20}\textbf{15.2}& \cellcolor{gray!20}99.7\\
\end{tabular}
}
\caption{Impact on the OOD results of the choice of the evaluation set in Argoverse 2 dataset ($\dagger$ means that the 2-stage MLP uses the annotation of unknown classes for its training). \todo{Test JE}}
\label{tab:eval_subset_setting_test_JE}
\end{table}
